Atomic Learning Objectives Labeling: A High-Resolution Approach for Physics Education

This paper introduces a novel approach to create a high-resolution "map" for physics learning: an "atomic" learning objectives (LOs) system designed to capture detailed cognitive processes and concepts required for problem solving in a college-level introductory physics course. Our method leverages Large Language Models (LLMs) for automated labeling of physics questions and introduces a comprehensive set of metrics to evaluate the quality of the labeling outcomes. The atomic LO system, covering nine chapters of an introductory physics course, uses a "subject-verb-object'' structure to represent specific cognitive processes. We apply this system to 131 questions from expert-curated question banks and the OpenStax University Physics textbook. Each question is labeled with 1-8 atomic LOs across three chapters. Through extensive experiments using various prompting strategies and LLMs, we compare automated LOs labeling results against human expert labeling. Our analysis reveals both the strengths and limitations of LLMs, providing insight into LLMs reasoning processes for labeling LOs and identifying areas for improvement in LOs system design. Our work contributes to the field of learning analytics by proposing a more granular approach to mapping learning objectives with questions. Our findings have significant implications for the development of intelligent tutoring systems and personalized learning pathways in STEM education, paving the way for more effective "learning GPS'' systems.

==> tables/Q_class_dist.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cc}
\toprule
\multicolumn{2}{c}{\textbf{Math Content Classifications}} \\
\midrule
\textbf{Classification} & \textbf{Questions} \\
\midrule
Algebra & 315 \\
Number \& Operation & 312 \\
Geometry \& Measurement & 122 \\
Probability & 44 \\
Data Analysis & 14 \\
\bottomrule
\toprule
\multicolumn{2}{c}{\textbf{Reading Content Classifications}} \\
\midrule
\textbf{Classification} & \textbf{Questions} \\
\midrule
Informational Text & 190 \\
Literature & 100 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{Distribution of questions across content classifications.}
\vspace{-2mm}
\label{tab:content_distribution}
\end{table}

==> tables/content_analysis.tex <==
\begin{figure}[t]
\centering
% \begin{minipage}[t]{0.50\linewidth}
% \begin{center}
\includegraphics[width=1\linewidth]{figures/content.png} 
% \end{center} 
% \end{minipage}
\hfill
\vspace{-5mm}
\caption{An illustration of MIA performance for LLMs across five math content classifications (Number \& Operation, Algebra, Geometry \& Measurement, Data Analysis, Probability) and two reading content classifications (Informational Text, Literature).}
\vspace{-3mm}
\label{figcontent}
\end{figure}

==> tables/cot.tex <==
\begin{table*}[t!]
\centering
\begin{minipage}[t]{0.9\textwidth}
\begin{lstlisting}[mathescape=true,basicstyle=\ttfamily\smalltonormalsize]
$\textbf{CoT Prompt for Malgorithm Identification}$: 

System: $\colorbox{lightyellow}{Provide step-by-step reasoning}$ to determine the answer rationale that corresponds to the given choice for the question. Then, provide your answer in the specified JSON format.

Question: {question}
Choice: {choice}
Answer Rationales:
{formatted_rationales}

Given the question and answer rationales, determine which answer rationale corresponds to the given choice for the question. 
$\colorbox{lightyellow}{Provide step-by-step reasoning. Show the steps.}$
And then provide your answer in the following JSON format:
{{
  "Correct Choice": "[A/B/C/D]"
}}
\end{lstlisting}
\end{minipage}
\caption{Prompt for the Malgorithm Identification experiment, where the LLM identifies the relationship between answer choices and rationales in a multiple-choice question-answering setting. The task involves identifying a "malgorithm", a rationale that represents flawed reasoning leading to an incorrect answer choice. The prompt provides the question, an answer choice (either correct or incorrect), and all rationales, asking the LLM to identify the rationale corresponding to the given choice. The highlighted sentence instructs the model to provide step-by-step reasoning, an instruction added for the Chain-of-Thought prompting strategy.}
\label{tab:cot_prompts}
\end{table*}


==> tables/dok_analysis.tex <==
\begin{figure*}[t!]
% \centering
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/math_dok.png} 
% \caption{r1}
% \label{dok1}
\end{center} 
\end{minipage}
\hfill
% \vspace{0.2 cm}
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/reading_dok.png} 
% \caption{r1}
% \label{dok2}
\end{center}
\end{minipage}
\caption{An illustration of MIA performance across different Grades and DOK levels for Math and Reading question sets. The top number represents MIA performance and the bottom number represents question counts. DOK I and II are selected for Math and DOK II and III for Reading. (best viewed in colors).}
\label{dok}
\end{figure*}

==> tables/dok_each.tex <==
\begin{figure*}[t!]
% \centering
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/number_dok.png} 
% \caption{r1}
% \label{dok1}
\end{center} 
\end{minipage}
\hfill
% \vspace{0.2 cm}
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/geometry_dok.png} 
% \caption{r1}
% \label{dok2}
\end{center}
\end{minipage}
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/algebra_dok.png} 
% \caption{r1}
% \label{dok1}
\end{center} 
\end{minipage}
\hfill
% \vspace{0.2 cm}
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/data_dok.png} 
% \caption{r1}
% \label{dok2}
\end{center}
\end{minipage}
\caption{An image of MIA performance across different Grades and DOK levels for various Content Classifications for Math question sets. The top number represents MIA performance and the bottom number represents question counts. The data analysis and probability classifications are combined together for illustration. (best viewed in colors).}
\label{math_dok_each}
\end{figure*}

==> tables/dok_each_reading.tex <==
\begin{figure*}[t!]
% \centering
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/information_dok.png} 
% \caption{r1}
% \label{dok1}
\end{center} 
\end{minipage}
\hfill
% \vspace{0.2 cm}
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/literature_dok.png} 
% \caption{r1}
% \label{dok2}
\end{center}
\end{minipage}
\caption{An image of MIA performance across different Grades and DOK levels for two Content Classifications for Reading question sets. The top number represents MIA performance and the bottom number represents question counts (best viewed in colors).}
\label{reading_dok_each}
\end{figure*}

==> tables/grade_content.tex <==
\begin{figure*}[t!]
% \centering
% \begin{minipage}[t]{0.7\linewidth}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/grade_content_math.png} 
% \caption{r1}
% \label{dok1}
\end{center} 
% \end{minipage}
\hfill
% \vspace{0.2 cm}
% \begin{minipage}[t]{0.55\linewidth}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/grade_content_reading.png}
% \label{dok2}
\end{center}
% \end{minipage}
\caption{An illustration of MIA performance across different Grades and Content Classifications for Math and Reading question sets. The top number represents MIA performance and the bottom number represents question counts (best viewed in colors).}
\label{grade_content}
\end{figure*}

==> tables/grade_level_dist.tex <==
\begin{table*}[t]
\begin{minipage}{.49\linewidth}
\begin{tabular}{cccc}
\toprule
\textbf{Subject} & \textbf{Grade} & \textbf{GPT 4o} & \textbf{LLaMA3-70B}\\
\midrule
\multirow{7}{*}{\textbf{Math}} & 3  & \underline{67.00} & 44.26 \\
& 4  & \underline{65.93} & \underline{54.13} \\
& 5  & \underline{66.52}  & 46.97 \\
& 6  & \underline{67.80} & \underline{58.84} \\
& 7  & 64.50 & \underline{57.49} \\
& 8  & 62.96 & 42.44 \\
& 11 & 53.68  & 41.03  \\
\midrule
& average & 65.10 & 50.60\\
\bottomrule
\end{tabular}
\end{minipage}
\begin{minipage}{.49\linewidth}
\begin{tabular}{cccc}
\toprule
\textbf{Subject} & \textbf{Grade} & \textbf{GPT 4o} & \textbf{LLaMA3-70B}\\
\midrule
\multirow{7}{*}{\textbf{Reading}} & 3  & \underline{73.81} & \underline{65.18} \\
& 4  & \underline{68.89} &  \underline{60.71} \\
& 5  & \underline{69.47}  & 45.68 \\
& 6  & 58.62 & 50.00 \\
& 7  & 63.46 & \underline{80.22} \\
& 8  & \underline{80.67} & \underline{62.00} \\
& 10 & 64.96  &  46.83 \\
\midrule
& average & 68.63 & 58.40 \\
\bottomrule
\end{tabular}
\end{minipage}
\caption{Grade-level performance distribution (MIA) for GPT-4o and LLaMA3-70B models using Chain-of-Thought prompting (few-shot for Math, zero-shot for Reading). Grades with above-average performance are \underline{\textbf{underlined}}.}
\label{tab:grade_score}
\end{table*}

==> tables/math_examples.tex <==
\begin{table*}[ht!]
\centering
\begin{tcolorbox}[colback=gray!10, colframe=gray!80!black,title=\textbf{\large Question}]
\large Each side of a square is 3 inches long. A student increases the length of each side by 3 inches. The area of the new square is how many times the area of the original square?
\end{tcolorbox}

% colback=blue!10, colframe=blue!80!black
% colback=teal!10, colframe=teal!80!black
% colback=blue!5,colframe=blue!40
% \begin{tcolorbox}[colback=green!5,colframe=green!40,title=\textbf{Answer Choices}]
% \begin{tcolorbox}[colback=,colframe=cyan!80!black,title=\textbf{\large Answer Choices}]
\begin{tcolorbox}[colback=navyblue!10,colframe=navyblue,title=\textbf{\large Answer Choices}]

\begin{enumerate}[label=(\Alph*)]
\item 9 (\normalsize Rationale: Squared the change in the length.)
\item 2 (\normalsize Rationale: Calculated the relationship between the sides.)
\item 3 (\normalsize Rationale: Used the change in the length.)
\item 4 (\normalsize Rationale: Calculated the area of the original square: $3 \times 3 = 9$ and the area of the new square with each side length increased by 3 inches: $6 \times 6 = 36$. Then determined that the area of the new square is 4 times the area of the original square.)
% \item 9 (\normalsize Malgorithm: Squared the change in the length.)
% \item 2 (\normalsize Malgorithm: Calculated the relationship between the sides.)
% \item 3 (\normalsize Malgorithm: Used the change in the length.)
% \item 4 (\normalsize Algorithm: Calculated the area of the original square: $3 \times 3 = 9$ and the area of the new square with each side length increased by 3 inches: $6 \times 6 = 36$. Then determined that the area of the new square is 4 times the area of the original square.)
\end{enumerate}
\end{tcolorbox}

\caption{An example question from the MalAlgoQA dataset illustrating the Malgorithm Identification task. Each answer choice is associated with a rationale, representing the reasoning process that led to that answer. The task for the model is to correctly identify the rationale given a particular answer choice. For incorrect answer choices, the corresponding rationales are malgorithms, representing flawed reasoning processes and thereby evaluating the counterfactual reasoning abilities of LLMs.}
\label{tab:math_example}
\end{table*}


==> tables/math_full_malagoqa.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{cccccc}
\toprule
\textbf{LLM} & \textbf{Num Shots} & \textbf{Prompting} & \textbf{MCQ} & \textbf{AIA} & \textbf{MIA} \\
\midrule
GPT 4o  & 0 & Simple & 90.11 & 92.06 & 62.82 \\
GPT 4o  & 5 & Simple &  & 90.61 & 64.99 \\
GPT 4o  & 0 & CoT & 97.61 & 95.65 & 66.1 \\
GPT 4o  & 5 & CoT &  & 95.49 & 65.1 \\
\midrule
LLaMA-70B  & 0 & Simple & 73.83 & 94.31 & 50.22 \\
LLaMA-70B  & 5 & Simple &  & 93.65 & 48.31 \\
LLaMA-70B  & 0 & CoT & 90.72 & 95.47 & 55.32 \\
LLaMA-70B  & 5 & CoT &  & 95.89 & 50.6 \\
\hline
GPT 3.5  & 0 & Simple & 52.85 & 77.08 & 35.8 \\
GPT 3.5  & 5 & Simple &  & 76.85 & 34.61 \\
GPT 3.5  & 0 & CoT & 82.53 & 86.28 & 14.74 \\
GPT 3.5  & 5 & CoT &  & 81.87 & 17.06 \\
\midrule
LLaMA-8B  & 0 & Simple & 45.79 & 75.29 & 34.81 \\
LLaMA-8B  & 5 & Simple &  & 80.32 & 38.41 \\
LLaMA-8B  & 0 & CoT & 70.68 & 83.07 & 27.05 \\
LLaMA-8B  & 5 & CoT &  & 83.05 & 31.39 \\
\bottomrule
\end{tabular}
\caption{Results for Math subject in the Cause Identification task.}
\label{tab:math_results}
\end{table*}

==> tables/question_level.tex <==
\begin{figure*}[t!]
% \centering
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/question_math.png} 
% \caption{r1}
% \label{dok1}
\end{center} 
\end{minipage}
\hfill
% \vspace{0.2 cm}
\begin{minipage}[t]{0.50\linewidth}
\begin{center}
\includegraphics[width=1\linewidth]{figures/question_reading.png} 
% \caption{r1}
% \label{dok2}
\end{center}
\end{minipage}
\caption{The distribution of GPT4-o performance in identifying malgorithms across question levels for math and reading question sets. The x-axis represents the number of correctly identified malgorithms per question, ranging from 0 to 3.}
\label{per-question}
\end{figure*}

==> tables/read_full_malagloqa.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|cccccc|}
% \toprule
\hline
\textbf{LLM} & \textbf{Num Shots} & \textbf{Prompting} & \textbf{MCQ} & \textbf{AIA} & \textbf{MIA} \\
\hline
GPT 4o  & 0 & Simple & 95.86 & 98.23 & 82.8 \\
GPT 4o  & 0 & CoT & 95.52 & 97.88 & 68.63 \\
\hline
LLaMA-70B  & 0 & Simple & 89.45 & 95.72 & 60.0 \\
LLaMA-70B  & 0 & CoT & 89.27 & 94.6 & 58.4 \\
\hline
GPT 3.5  & 0 & Simple & 84.83 & 95.05 & 13.98 \\
GPT 3.5  & 0 & CoT & 81.66 & 85.82 & 8.61 \\
\hline
LLaMA-8B  & 0 & Simple & 73.96 & 89.62 & 19.89 \\
LLaMA-8B  & 0 & CoT & 78.05 & 89.52 & 15.47 \\
\hline
% \bottomrule
\end{tabular}
\caption{Results for Reading subject in the Cause Identification task.}
\label{tab:reading_results}
\end{table*}

==> tables/results_full.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{ccccccc}
\toprule
\textbf{LLM} & \textbf{Subject} & \textbf{Num Shots} & \textbf{Prompting} & \textbf{MCQ} & \textbf{AIA} & \textbf{MIA} \\
\midrule
\multirow{2}{*}{GPT 4o}  & \multirow{2}{*}{Reading} & 0 & Simple & 95.86 & 98.23 & 82.80 \\
  &  & 0 & CoT & 95.52 & 97.88 & 68.63 \\
\midrule
\multirow{2}{*}{LLaMA3-70B}  & \multirow{2}{*}{Reading} & 0 & Simple & 89.45 & 95.72 & 60.00 \\
  &  & 0 & CoT & 89.27 & 94.60 & 58.40 \\
\midrule
\multirow{2}{*}{GPT-3.5}  & \multirow{2}{*}{Reading} & 0 & Simple & 84.83 & 95.05 & 13.98 \\
  &  & 0 & CoT & 81.66 & 85.82 & 8.61 \\
\midrule
\multirow{2}{*}{LLaMA3-8B}  & \multirow{2}{*}{Reading} & 0 & Simple & 73.96 & 89.62 & 19.89 \\
  &  & 0 & CoT & 78.05 & 89.52 & 15.47 \\
\bottomrule
\toprule
\multirow{4}{*}{GPT 4o}  & \multirow{4}{*}{Math} & 0 & Simple & 90.11 & 92.06 & 62.82 \\
 &  & 5 & Simple &  & 90.61 & 64.99 \\
  &  & 0 & CoT & 97.61 & 95.65 & 66.10 \\
  &  & 5 & CoT &  & 95.49 & 65.10 \\
\midrule
\multirow{4}{*}{LLaMA3-70B}  & \multirow{4}{*}{Math} & 0 & Simple & 73.83 & 94.31 & 50.22 \\
  &  & 5 & Simple &  & 93.65 & 48.31 \\
  &  & 0 & CoT & 90.72 & 95.47 & 55.32 \\
  &  & 5 & CoT &  & 95.89 & 50.6 \\
\midrule
\multirow{4}{*}{GPT 3.5}  & \multirow{4}{*}{Math} & 0 & Simple & 52.85 & 77.08 & 35.8 \\
&  & 5 & Simple &  & 76.85 & 34.61 \\
  &  & 0 & CoT & 82.53 & 86.28 & 14.74 \\
  &  & 5 & CoT &  & 81.87 & 17.06 \\
\midrule
\multirow{4}{*}{LLaMA3-8B}  & \multirow{4}{*}{Math} & 0 & Simple & 45.79 & 75.29 & 34.81 \\
 &  & 5 & Simple &  & 80.32 & 38.41 \\
 &  & 0 & CoT & 70.68 & 83.07 & 27.05 \\
 &  & 5 & CoT &  & 83.05 & 31.39 \\
\bottomrule
\end{tabular}
\caption{Performance results of different Large Language Models (LLMs) on the Malgorithm Identification task, presented separately for Reading and Math subjects. The results are organized according to the type of prompting (Simple or CoT), and the number of shots (0 or 5). The metrics evaluated include Multiple-Choice Question (MCQ) accuracy, Algorithm Identification Accuracy (AIA), and Malgorithm Identification Accuracy (MIA). AIA measures the model's ability to identify the correct rationale or algorithm that aligns with the given correct answer choice, whereas MIA measures the model's ability to identify the flawed reasoning or malgorithm that aligns with the given incorrect answer choice. It can be observed that achieving higher scores in MIA is generally more challenging than AIA, highlighting the complexity of counterfactual reasoning tasks.}
\label{tab:results}
\end{table*}

==> tables/simple_vs_cot.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|ccccc|}
\toprule
\textbf{LLM} & \textbf{Subject} & \textbf{Prompting} & \textbf{AIA} & \textbf{MIA} \\
\hline
GPT-4o & Math & CoT & 95.49 & 65.10 \\
       &      & Simple & 90.61 & 64.99 \\
       & Reading & CoT & 97.88 & 68.63 \\
       &      & Simple & 98.23 & 82.80 \\
\hline
LLaMA-70B & Math & CoT & 95.89 &	50.6 \\
          &      & Simple & 93.65	& 48.31 \\
          & Reading & CoT & 94.6 &	58.4 \\
          &      & Simple & 95.72	& 60.0 \\
\hline
\end{tabular}
\caption{Algorithm Identification Accuracy (AIA) and Malgorithm Identification Accuracy (MIA) for Math and Reading subjects in zero-shot setting.}
\label{tab:aia_mia}
\end{table*}
